SAPG: Split and Aggregate Policy Gradients

Despite extreme sample inefficiency, on-policy reinforcement learning, aka policy gradients, has become a fundamental tool in decision-making problems. With the recent advances in GPU-driven simulation, the ability to collect large amounts of data for RL training has scaled exponentially. However, we show that current RL methods, e.g. PPO, fail to ingest the benefit of parallelized environments beyond a certain point and their performance saturates. To address this, we propose a new on-policy RL algorithm that can effectively leverage large-scale environments by splitting them into chunks and fusing them back together via importance sampling. Our algorithm, termed SAPG, shows significantly higher performance across a variety of challenging environments where vanilla PPO and other strong baselines fail to achieve high performance. Website at https://sapg-rl.github.io/

==> archive.tex <==
\section{Background}
\paragraph{Problem setting} Reinforcement learning is generally applied to problems that are modeled as Markov Decision Processes. An MDP is characterized by a tuple ($\mathcal{S}, \mathcal{A}, \mathcal{P}, r, \rho, \gamma)$ where $\mathcal{S}$ is the set of states, $\mathcal{A}$ is the set of actions, $\mathcal{P}: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow \mathbb{R}$ encodes the transition probabilities, $r: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ represents the reward function. $\rho: \mathcal{S} \rightarrow \mathbb{R}$ represents the initial distribution of states and  $\gamma$ represents the discount factor.

The objective in reinforcement learning is to find a policy $\pi(a|s)$ which maximises the long term discounted reward 

\begin{equation}
\label{eq:rl_obj}
\mathcal{J}(\pi) = \mathop{\mathbb{E}}_{s_0 \sim \rho, a_t \sim \pi(\cdot|s_t) }\left[ \sum_{t=0}^{T-1} \gamma^tr(s_t, a_t)\right]
%s_{t+1} \sim \mathcal{P}(s_t, a_t, \cdot)
\end{equation}

For simplicity, we will state all subsequent equations assuming infinite horizon tasks i.e. $T = \infty$.

Two more quantities of interest are

\begin{align*}
  Q^{\pi}(s_t, a_t) &=  \mathop{\mathbb{E}}_{\pi}\left[r(s_t, a_t) + \sum_{i=1}^{\infty} \gamma^ir(s_{t+i}, a_{t+1})\right] \\
V^{\pi}(s_t) &=  \mathop{\mathbb{E}}_{\pi}\left[r(s_t, a_t) + \sum_{i=1}^{\infty} \gamma^ir(s_{t+i}, a_{t+1})\right] \\
&= \mathop{\mathbb{E}}_{a_t \sim \pi(s_t)}\left[Q^{\pi}(s_t, a_t)\right] 
\end{align*}

$Q^{\pi}(s_t, a_t)$, known as the Q-value, denotes the expected discounted reward if the agent starts from state $s_t$, executes action $a_t$ and then follows the policy $\pi$ after that. 
$V^{\pi}(s_t, a_t)$, known as the value function, denotes the expected discounted reward if the agent starts from state $s_t$ and follows the policy $\pi$.

\paragraph{On-policy reinforcement learning}
On-policy reinforcement learning tries to optimize the RL objective by iteratively improving it's estimate of the best policy. The most common class of on-policy reinforcement learning algorithms are policy-gradient algorithms.

Policy gradient algorithms try to maximize the objective $\mathcal{J}$ by performing some form of gradient descent on the objective function. One of the earliest such algorithms, REINFORCE \cite{reinforce} \todo{reinforce ref}
derives the gradient  of \eqref{eq:rl_obj} for a parameterized policy $\pi_\theta$ as follows
\begin{equation}
\nabla_{\theta} J(\pi_\theta) = \mathop{\mathbb{E}}_{s \sim \rho_d, a \sim \pi(\cdot| s)}\left[\nabla_{\theta}\log(\pi_\theta(a))Q^{\pi_\theta}(s,a)\right]
\end{equation}
where $\rho_d$ denote the discounted state visitation probability, $\rho_d(s) = \sum_{i=0}^T \gamma^t\mathbb{P}(s_{i} = s)$.

The above gradient is calculated using a Monte-Carlo estimate from a sample of trajectories. This leads to a high variance estimate and consequently unstable learning. A common technique applied to reduce this variance is learning a state-dependent baseline \cite{actorcritic}, which is generally an estimate of the value function $\hat{V}^{\pi_{\theta}}(s)$, and subtract it from $Q^{\pi_\theta}(s,a)$ to get 
\begin{equation}
\nabla_{\theta} J(\pi_\theta) = \mathop{\mathbb{E}}_{s \sim \rho_d, a \sim \pi(\cdot| s)}\left[\nabla_{\theta}\log(\pi_\theta(a))\hat{A}^{\pi_\theta}(s,a)\right]
\end{equation}
where $\hat{A}^{\pi_\theta}(s,a) = \hat{Q}^{\pi_\theta}(s,a) - \hat{V}^{\pi_{\theta}}(s)$, which is termed as the advantage. Here $\hat{Q}^{\pi_\theta}(s,a)$ the Monte Carlo estimate. To further reduce variance, instead of using Monte-Carlo, algorithms also use bootstrapped estimates of $\hat{Q}^{\pi_\theta}$ using the value function $\hat{V}^{\pi_{\theta}}$. \todo{Bootstrapping refs}

Since then, policy gradient methods have evolved to incorporate many more techniques such as natural policy gradients \cite{natural_pg, trpo}. Today, the most widely used policy gradient method is PPO \cite{ppo}, whose loss for gradient update is as follows
\begin{equation}
\label{eq:ppo_loss}
L(\pi_\theta) = \mathop{\mathbb{E}}_{\pi_{old}}\left[ \min(r_t(\pi_\theta), \mathop{clip}(r_t(\pi_\theta), 1 - \epsilon, 1+ \epsilon))A_t^{\pi_{old}}\right]   
\end{equation}
Here, $r_t(\pi_\theta) = \frac{\pi_{\theta}(a_t|s_t)}{\pi_{old}(a_t|s_t)}$ and $\pi_{old}$ is the policy collecting the on-policy data. 
Something to note here is that, after update step with this loss function, subsequent update steps with more minibatches are off-policy i.e. the data is already outdated. The fact that PPO is able to learn despite this makes way for off-policy updates in PPO.

\paragraph{Off-policy update}

\cite{off-policy-ppo} introduce an off-policy version of PPO where $\pi_{old}$ is replaced by a behaviour policy $\mu$ in \eqref{eq:ppo_loss}. The advantage estimates are also updated accordingly using the current value function $V^{\pi_{\theta}}$. The new loss function looks like 

\begin{multline}
\label{eq:offp_ppo_loss}
L_{off-policy}(\pi_\theta) = \mathop{\mathbb{E}}_{\mu}\left[ \min(\frac{\pi_{\theta}(a_t|s_t)}{\mu(a_t|s_t)}, \right.\\
\left.\mathop{clip}(\frac{\pi_{\theta}(a_t|s_t)}{\mu(a_t|s_t)}, 1 - \epsilon, 1+ \epsilon))A_t^{\pi_{old}}(s_t, a_t)\right]   
\end{multline}

\cite{off-policy-ppo} use a V-trace target \cite{vtrace} to compute the advantage $A_t^{\pi_{old}}(s_t, a_t)$ estimates. However, as will be described later, we combine off-policy data and on-policy data and use single-step estimates of $A_t^{\pi_{old}}(s_t, a_t)$ using the current value network $V^{\pi_{\theta}}(s_t, a_t)$. Our loss function is a simple sum of \eqref{eq:offp_ppo_loss} and \eqref{eq:ppo_loss}.

\section{The Method}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,height=5cm]{example-image-a}
    \caption{Our method}
    \label{fig:method}
\end{figure*}
Observing that simply increasing the data throughput does not help scale PPO to learn on hard manipulation environments,
the core idea behind our method is combining data from different policies in an on-policy style update. The detailed description of the method is given below.

We train $M$ different policies $\pi_1,\pi_2,\pi_3,...\pi_M$ where all policies share the same network parameterized by $\theta$ and differ only by a \textbf{learned} parameter vector $\mathbf{l}_i$ private to each policy that is concatenated with the input observation to the policy. Thus, each policy differs only by the values in the learned parameter vector. Note that, by policy, we mean both the actor $\pi_{\theta}$ and the value networks $V_{\theta}$. Thus, $\pi_i(s,a) = \pi_\theta(a|s,\mathbf{l}_j)$.


We partition $N\times M$ IsaacGym environments into M blocks each with N environment instances. The $i^{th}$ block corresponds to environments for use for rolling out the policy $\pi_i$. Each policy is rolled out for $k$ steps in it's environments between each network update. Thus, in this case the loss formulation for PPO would be

\begin{multline}
\label{lp_pp_loss}
L(\theta) = \mathop{\mathbb{E}}_{(s_t^j, a_t^j) \sim \pi_j}\left[ \sum_{j=1}^{M}\min(\frac{\pi_{\theta}(a_t^j|s_t^j,\mathbf{l}_j)}{\pi_{\theta_{old}}(a_t^j|s_t^j,\mathbf{l}_j)}, \right. \\
\left.\mathop{clip}(\frac{\pi_{\theta}(a_t^j|s_t^j,\mathbf{l}_j)}{\pi_{\theta_{old}}(a_t^j|s_t^j,\mathbf{l}_j)}, 1 - \epsilon, 1+ \epsilon))A_{t,\theta_{old}}^{j}\right] 
\end{multline}

where $A_{t,\theta_{old}}^{j} = \sum_{k=t}^{t+d - 1}\gamma^{k-j}r_k^j + \gamma^dV_{\theta}(s_{t+d}^j, \mathbf{l}_j) - V_{\theta}(s_t^j, \mathbf{l}_j)$ 
After obtaining a batch of data from the rollout, we perform what we call off-policy combination. We relabel data from a random policy $\pi_j \neq \pi_1$ to behave like data from $\pi_i$ by exchanging the parameters concatenated with observation and updating the advantages to correspond to the value network for $\pi_1$. Let $V_\theta$ denote value network, and $(s_t^j, a_t^j, r_t^j, s_{t+1}^j)$ denote data from policy $\pi_j$. The off-policy advantage calculation is as follows - 

\begin{equation}
    A_{t,\theta}^{i}(s_t^j, a_t^j) = r_t^j + V_{\theta}(s_t^j, \mathbf{l}_1) - V_{\theta}(s_{t+1}^j,\mathbf{l}_1)
\end{equation}

This serves as off policy data for $\pi_1$.
Thus, $\pi_1$ behaves like a "leader" which obtains data from itself in addition to off-policy data from others while other policies behave like "follower" policies learn through their own data and as well as feeding data into the leader. 

The efficiency in data usage is two-fold. We update a shared network which to help data collected by all policies to contribute to learning while also sourcing data from "followers" to create off-policy data for the leader, which will be our final policy for evaluation.

\subsection{Encouraging exploration}

We also test a version of our method that explicitly encourages varied degrees exploration of exploration with different policies. Instead of the "follower" policies being just different policies following the same training procedure as the leader, we train each of them with a different entropy coefficient $c_j$ to encourage exploration while the "leader" policy is assigned an entropy coefficient of $c_1=0$ and receives exploration data from the "followers" through off-policy combination. We add the follow term to the loss

\begin{equation}
    L_{ent} = -\frac{1}{M}\sum_{j=1}^{M}c_j\mathcal{H}(\pi_j(s_t^j))
\end{equation}

Note that, in our implementation for this case, $\pi_{\theta}$ is implemented as a Gaussian policy with an feedforward network $\mu_\theta$ which takes as input $(s_t^j,l_j)$ while $\sigma_\theta$ is implemented using a collection of M learned vectors $\{\boldsymbol{\sigma}_i\}_{i=1}^M$. Thus,

\begin{equation}
    \pi_{\theta}(s, \mathbf{l}_j) = (\mu_{\theta}(s,l_j),\boldsymbol{\sigma}_j)
\end{equation}


